Complexity of the General Chromatic Art Gallery Problem

In the original Art Gallery Problem (AGP), one seeks the minimum number of guards required to cover a polygon $P$. We consider the Chromatic AGP (CAGP), where the guards are colored. As long as $P$ is completely covered, the number of guards does not matter, but guards with overlapping visibility regions must have different colors. This problem has applications in landmark-based mobile robot navigation: Guards are landmarks, which have to be distinguishable (hence the colors), and are used to encode motion primitives, \eg, "move towards the red landmark". Let $\chi_G(P)$, the chromatic number of $P$, denote the minimum number of colors required to color any guard cover of $P$. We show that determining, whether $\chi_G(P) \leq k$ is \NP-hard for all $k \geq 2$. Keeping the number of colors minimal is of great interest for robot navigation, because less types of landmarks lead to cheaper and more reliable recognition.

==> Makefile <==
LANGUAGE = en_US
DOCUMENTS = main.pdf
TEXFILES := $(sort $(wildcard *.tex))

PDFLATEX = pdflatex
PDFLATEXFLAGS = -halt-on-error -file-line-error
BIBTEX = bibtex
BIBTEXFLAGS =

#GRAPHICS_STATIC = $(foreach g, \
#	prototyp.pdf, \
#	pics/$g)

GRAPHICS_STATIC =

GRAPHICS_PDF =

GRAPHICS_PDFTEX = $(foreach g, \
	3sat gadget_and gadget_crossing_2 gadget_inverter gadget_multiplexer \
	gadget_or_bb gadget_or_rb gadget_variable needles three_colorability, \
	graphics/$g.pdf_tex)

main.pdf: main.tex eurocg14.cls \
	abs2.tex \
	intro2.tex \
	preliminaries.tex \
	three2.tex \
	two-colorability.tex \
	simple.tex \
	conclusion.tex \
	bibliography.bib
#	$(GRAPHICS_STATIC) $(GRAPHICS_PDF) $(GRAPHICS_PDFTEX)

.DEFAULT_GOAL = all
.PHONY: all todo spellcheck clean

all: $(DOCUMENTS)

todo:
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		grep -hnT TODO $$texfile || true; \
		grep -hnTo '\\\(todo\|missingfigure\)\(\[.*\]\)\?{.*}' $$texfile | detex || true; \
	done

spellcheck:
	for texfile in $(TEXFILES); do \
		aspell --lang=$(LANGUAGE) check $$texfile; \
	done

$(DOCUMENTS): %.pdf: %.tex
	$(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}
	if grep -e '\citation' -e '\bibdata' -e '\bibstyle' *.aux; then \
		$(BIBTEX) $(BIBTEXFLAGS) $* && $(PDFLATEX) $(PDFLATEXFLAGS) \\input{$<}; \
	fi
	$(PDFLATEX) $(PDFLATEXFLAGS) -recorder \\input{$<}
	grep '^OUTPUT ' $*.fls \
		| sed -e 's/^OUTPUT //' \
		| grep -vx $@ \
		| xargs rm
	rm $*.fls
	rm -f $*.bbl $*.blg

%.ps: %.pdf
	pdf2ps -dLanguageLevel=3 $< $@

$(GRAPHICS_PDF): %.pdf: %.svg
	inkscape --without-gui --export-pdf=$*.pdf $*.svg

$(GRAPHICS_PDFTEX): %.pdf_tex: %.svg
	inkscape --without-gui --export-latex --export-pdf=$*.pdf $*.svg

clean:
	rm -f $(DOCUMENTS) main.dvi make.log
#	rm -f $(GRAPHICS_PDF)
#	rm -f $(GRAPHICS_PDFTEX)
#	rm -f $(GRAPHICS_PDFTEX:.pdf_tex=.pdf)


==> abstract.tex <==
\begin{abstract}
In the original Art Gallery Problem (AGP), one seeks the minimum number of guards required to cover a polygon $P$.
We consider the Chromatic AGP (CAGP), where the guards are colored.
As long as $P$ is completely covered, the number of guards does not matter, but guards with overlapping visibility regions must have different colors.
This problem has applications in landmark-based mobile robot navigation:
Guards are landmarks, which have to be distinguishable (hence the colors), and are used to encode motion primitives, \eg, ``move towards the red landmark''.
Let $\chi_G(P)$, the chromatic number of $P$, denote the minimum number of colors required to color any guard cover of $P$.
We show that determining, whether $\chi_G(P) \leq k$ is \NP-hard for all $k \geq 2$.
Keeping the number of colors minimal is of great interest for robot navigation, because less types of landmarks lead to cheaper and more reliable recognition.
\end{abstract}


==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}

The \textsc{Art Gallery Problem} (AGP) is a classical problem.
Given a polygon $P$ with $n$ vertices, how many point-shaped, immobile guards does it take to cover all of $P$, \ie, to make sure that every point in $P$ is seen by at least one guard?
As first shown by Chvátal~\cite{c-ctpg-75} and elegantly shown by Fisk~\cite{f-spcwt-78}, up to $\left\lfloor \frac{n}{3} \right\rfloor$ guards are sometimes necessary and always sufficient.
The AGP is \NP-hard~\cite{ll-ccagp-86} and has received a significant amount of attention ever since, including theoretical insights (consult~\cite{r-agta-87,s-rrag-92,u-agip-00} for an overview), as well as, more recently, practical results (\cite{kbfs-esbgagp-12,trs-tqfosftagpapia-13,ffks-ffagp-13b} to name a few).

We study a variant of the AGP called the \textsc{Chromatic AGP} (CAGP).
The objective is to find a set of guards covering $P$, such that two guards which see the same spot are in \emph{conflict} and need a different color.
The problem was first introduced by Erickson et~al.~\cite{el-acagp-10} and originates from the field of robot navigation:
A mobile robot's course through the polygonal landscape $P$ is plotted using landmarks (guards) to formulate motion primitives, \eg: ``move toward the landmark~1, while keeping a constant distance to landmark~2''.
Landmarks can be optical features or radio signals.
For this kind of navigation, the robot must always see some landmark, which is why the CAGP asks for a guard cover of $P$, and it should never see two indistinguishable landmarks, hence the requirement of a non-conflicting guard cover.
The number of colors is minimized, because distinguishing only a few types of landmarks is much easier on the pattern-recognition level~\cite{el-aagatetlad-11}.
A resulting question is, how many colors are needed for any guard cover of $P$, which Erickson et~al. called the \emph{chromatic art gallery number} $\chi_G(P)$.
Note that in the CAGP it is not necessary to minimize the cardinality of a guard cover, only the number of colors.
Erickson et~al. established upper and lower bounds for general polygons as well as special classes of polygons~\cite{el-acagp-10,el-aagatetlad-11,el-hmlcantaciap-11}.

Many of those bounds state that occasionally a large number of colors is required.\todo{details}{}
Motivated by those numbers, Bärtschi et~al. introduced the \textsc{Conflict Free CAGP}, where they relax the chromatic requirements~\cite{bs-cfcagc-12}:
Visibility regions of guards with the same color may overlap, as long as there is always one uniquely colored guard visible.

Erickson et~al. proved that choosing a colored guard cover with a minimum number of colors \emph{from a fixed set of candidates} in simple polygon is \NP-hard~\cite{el-hmlcantaciap-11}.
Their proof is based on that of the \NP-hardness of the original AGP by Lee et~al.~\cite{ll-ccagp-86} and does not generalize to our contribution.\todo{check}

\paragraph{Our Contribution}

Our main result is to show the \NP-hardness for arbitrary polygons \emph{without} a fixed set of guard candidates:
Let $k$-CAGP denote the decision problem whether a colored guard cover with no more than $k$ colors exists for a polygon $P$, \ie, if $\chi_G(P) \leq k$.
Section~\ref{sec:preliminaries} contains definitions and basic lemmas, Section~\ref{sec:three-colorability} gives an easy proof that $k$-CAGP is \NP-hard for $k = 3$, which is generalized to $k \geq 3$.
Our main result is presented in Section~\ref{sec:two-colorability}:
$2$-CAGP is \NP-hard as well.
Section~\ref{sec:conclusion} concludes this paper.


==> three-colorability.tex <==
\section{3- and (3+k)-Colorability}
\label{sec:three-colorability}

This section provides an easy proof for the \NP-hardness of $3$-CAGP, which is then generalized for $(3+k)$-CAGP with $k \geq 1$.

\subsection{3-Colorability}

Let $3$-PGC denote the following decision problem:
Given a planar graph $H$, is its chromatic number $3$ or less?
$3$-PGC is known to be \NP-complete~\cite{gj-cai-79}.

We infer the \NP-hardness of $3$-CAGP from that of $3$-PGC, but skip details due to space restrictions.
The reduction principle is depicted by the continuous lines in Figure~\ref{fig:3color}:
Each node of the graph $H$ is turned into a convex region of the polygon $P$, and needles force exactly one guard into each of them by Lemma~\ref{lem:needles}.
Those guards cover $P$; it is easy to see that $P$ is $3$-colorable iff $H$ is $3$-colorable, because the edges of $H$ are translated into tunnels with a turn in the middle, preventing adjacent vertex gadgets' guards from sharing identical colors.

\begin{figure}
  \begin{center}
    \def\svgwidth{0.9\textwidth}
    \input{graphics/three_colorability.pdf_tex}
  \end{center}
  \caption{$3$- and $(3+k)$-colorability.
    $3$-colorability is shown in continuous lines, $(3+k)$-colorability is achieved by adding the structures drawn in dashed lines.
    The gray areas contain $k$ or $3$ forced guards.}
  \label{fig:3color}
\end{figure}

\subsection{(3+k)-Colorability}
\label{sec:k-colorability}

For $1 \leq k \in \N$, the reduction of $3$-PGC to $3$-CAGP can be generalized to $(3+k)$-CAGP by adding the structures drawn in dashed lines to Figure~\ref{fig:3color}.
Extra gadgets with $k$ forced guards (by Lemma~\ref{lem:needles}) are added for each face of $H$.
Those gadgets' colors are synchronized by connecting tunnels with a group of $3$ guards behind a turn (similar to the inverter gadget in Section~\ref{sec:inverter-gadget}), and thus globally consume $k$ of the $3+k$ available colors.
The crossing of the gadget connections with the tunnels corresponding to the original edges of $G$ enforce the rest of $P$ to be colored, using only the remaining $3$ colors.
Hence, $P$ is $(3+k)$-colorable iff $H$ is $3$-colorable.

